Forward pi+/- production in p-O2 and p-N2 interactions at 12 GeV/c

Measurements of double-differential charged pion production cross-sections in interactions of 12 GeV/c protons on O_2 and N_2 thin targets are presented in the kinematic range 0.5 GeV/c < p_{\pi} < 8 GeV/c and 50 mrad < \theta_{\pi} < 250 mrad (in the laboratory frame) and are compared with p--C results. For p--N_2 (p--O_2) interactions the analysis is performed using 38576 (7522) reconstructed secondary pions. The analysis uses the beam instrumentation and the forward spectrometer of the HARP experiment at CERN PS. The measured cross-sections have a direct impact on the precise calculation of atmospheric neutrino fluxes and on the improved reliability of extensive air shower simulations by reducing the uncertainties of hadronic interaction models in the low energy range. In particular, the present results allow the common hypothesis that p--C data can be used to predict the p--N_2 and p--O_2 pion production cross-sections to be tested.

==> data_table.tex <==
\begin{appendix}

\section{Cross-section data}\label{app:data}

\begin{table}[!h]
  \caption{\label{tab:xsec_results_pC12_pip_pim_2}
    HARP results for the double-differential $\pi^+$ and $\pi^-$ production
    cross-section in the laboratory system,
    $d^2\sigma^{\pi}/(dpd\Omega)$, for p-C interactions at 12~\GeVc. 
    Each row refers to a
    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
    The central value as well as the square-root of the diagonal elements
    of the covariance matrix are given.}
  \centerline{
    \input{tables/xsec_results_pC12_pip_pim_1.tex}
  }
  %\caption{\label{tab:xsec_results1}
  %  HARP results for the double-differential $\pi^+$ production
  %  cross-section in the laboratory system,
  %  $d^2\sigma^{\pi^+}/(dpd\Omega)$. Each row refers to a
  %  different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
  %  \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
  %  where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
  %  The central value as well as the square-root of the diagonal elements
  %  of the covariance matrix are given.}
\end{table}

\begin{table}
  \centerline{
    \input{tables/xsec_results_pC12_pip_pim_2.tex}
  }
\end{table}


%\begin{table}[!h]
%  \caption{\label{tab:xsec_results_pC12_pim_2}
%    HARP results for the double-differential $\pi^-$ production
%    cross-section in the laboratory system,
%    $d^2\sigma^{\pi^-}/(dpd\Omega)$, for p-C interactions at 12~\GeVc. 
%    Each row refers to a
%    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
%    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
%    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
%    The central value as well as the square-root of the diagonal elements
%    of the covariance matrix are given.}
%  \centerline{
%    \input{tables/xsec_results_pC12_pim_1.tex}
%  }
  %\caption{\label{tab:xsec_results1}
  %  HARP results for the double-differential $\pi^+$ production
  %  cross-section in the laboratory system,
  %  $d^2\sigma^{\pi^+}/(dpd\Omega)$. Each row refers to a
  %  different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
  %  \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
  %  where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
  %  The central value as well as the square-root of the diagonal elements
  %  of the covariance matrix are given.}
%\end{table}
%
%\begin{table}
%  \centerline{
%    \input{tables/xsec_results_pC12_pim_2.tex}
%  }
%\end{table}



\begin{table}
  \caption{\label{tab:xsec_results_pipC12_pip_pim_1}
    HARP results for the double-differential $\pi^+$ and $\pi^-$ production
    cross-section in the laboratory system,
    $d^2\sigma^{\pi}/(dpd\Omega)$, for \pip-C interactions at 12~\GeVc. 
    Each row refers to a
    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
    The central value as well as the square-root of the diagonal elements
    of the covariance matrix are given.}
  \centerline{
    \input{tables/xsec_results_pipC12_pip_pim_1.tex}
  }
\end{table}

%\begin{table}
%  \caption{\label{tab:xsec_results_pipC12_pim_1}
%    HARP results for the double-differential $\pi^-$ production
%    cross-section in the laboratory system,
%    $d^2\sigma^{\pi^-}/(dpd\Omega)$, for \pip-C interactions at 12~\GeVc. 
%    Each row refers to a
%    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
%    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
%    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
%    The central value as well as the square-root of the diagonal elements
%    of the covariance matrix are given.}
%  \centerline{
%    \input{tables/xsec_results_pipC12_pim_1.tex}
%  }
%\end{table}


\begin{table}
  \caption{\label{tab:xsec_results_pimC12_pip_pim_1}
    HARP results for the double-differential $\pi^+$ and $\pi^-$ production
    cross-section in the laboratory system,
    $d^2\sigma^{\pi}/(dpd\Omega)$, for \pim-C interactions at 12~\GeVc. 
    Each row refers to a
    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
    The central value as well as the square-root of the diagonal elements
    of the covariance matrix are given.}
  \centerline{
    \input{tables/xsec_results_pimC12_pip_pim_1.tex}
  }
\end{table}

%\begin{table}
%  \caption{\label{tab:xsec_results_pimC12_pim_1}
%    HARP results for the double-differential $\pi^-$ production
%    cross-section in the laboratory system,
%    $d^2\sigma^{\pi^-}/(dpd\Omega)$, for \pim-C interactions at 12~\GeVc. 
%    Each row refers to a
%    different $(p_{\hbox{\small min}} \le p<p_{\hbox{\small max}},
%    \theta_{\hbox{\small min}} \le \theta<\theta_{\hbox{\small max}})$ bin,
%    where $p$ and $\theta$ are the pion momentum and polar angle, respectively.
%    The central value as well as the square-root of the diagonal elements
%    of the covariance matrix are given.}
%  \centerline{
%    \input{tables/xsec_results_pimC12_pim_1.tex}
%  }
%\end{table}

\end{appendix}


==> xsec_results_pC12_pip_1.tex <==
\begin{tabular}{|c|c|c|c|rcr|} \hline
$\theta_{\hbox{\small min}}$ &
$\theta_{\hbox{\small max}}$ &
$p_{\hbox{\small min}}$ &
$p_{\hbox{\small max}}$ &
\multicolumn{3}{c|}{$d^2\sigma^{\pi^+}/(dpd\Omega)$} 
\\
(mrad) & (mrad) & (GeV/c) & (GeV/c) &
\multicolumn{3}{c|}{(mb/(GeV/c sr))}
\\ \hline
%
 30 &  60 & 0.5 & 1.0 & $198.5$ & $\pm$ & $40.8$ \\
    &     & 1.0 & 1.5 & $245.8$ & $\pm$ & $35.0$ \\
    &     & 1.5 & 2.0 & $248.2$ & $\pm$ & $31.1$ \\
    &     & 2.0 & 2.5 & $227.9$ & $\pm$ & $31.0$ \\
    &     & 2.5 & 3.0 & $331.6$ & $\pm$ & $34.2$ \\
    &     & 3.0 & 3.5 & $258.2$ & $\pm$ & $31.4$ \\
    &     & 3.5 & 4.0 & $214.1$ & $\pm$ & $30.5$ \\
    &     & 4.0 & 5.0 & $133.5$ & $\pm$ & $15.1$ \\
    &     & 5.0 & 6.5 & $102.6$ & $\pm$ & $11.0$ \\
    &     & 6.5 & 8.0 & $45.2$ & $\pm$ & $7.8$ \\ \hline

 60 &  90 & 0.5 & 1.0 & $191.7$ & $\pm$ & $29.1$ \\
    &     & 1.0 & 1.5 & $243.2$ & $\pm$ & $25.4$ \\
    &     & 1.5 & 2.0 & $284.9$ & $\pm$ & $27.9$ \\
    &     & 2.0 & 2.5 & $284.4$ & $\pm$ & $24.3$ \\
    &     & 2.5 & 3.0 & $214.9$ & $\pm$ & $19.8$ \\
    &     & 3.0 & 3.5 & $163.1$ & $\pm$ & $15.8$ \\
    &     & 3.5 & 4.0 & $148.4$ & $\pm$ & $15.2$ \\
    &     & 4.0 & 5.0 & $91.4$ & $\pm$ & $9.3$ \\
    &     & 5.0 & 6.5 & $36.9$ & $\pm$ & $5.0$ \\
    &     & 6.5 & 8.0 & $15.6$ & $\pm$ & $2.7$ \\ \hline

 90 &  120 & 0.5 & 1.0 & $204.0$ & $\pm$ & $27.8$ \\
    &     & 1.0 & 1.5 & $243.7$ & $\pm$ & $26.2$ \\
    &     & 1.5 & 2.0 & $269.4$ & $\pm$ & $27.7$ \\
    &     & 2.0 & 2.5 & $221.3$ & $\pm$ & $23.4$ \\
    &     & 2.5 & 3.0 & $168.0$ & $\pm$ & $17.0$ \\
    &     & 3.0 & 3.5 & $140.5$ & $\pm$ & $15.2$ \\
    &     & 3.5 & 4.0 & $94.8$ & $\pm$ & $15.6$ \\
    &     & 4.0 & 5.0 & $50.2$ & $\pm$ & $6.3$ \\
    &     & 5.0 & 6.5 & $18.0$ & $\pm$ & $2.9$ \\
    &     & 6.5 & 8.0 & $4.7$ & $\pm$ & $1.2$ \\ \hline
\end{tabular}


